A Categorical Unification for Multi-Model Data: Part II Categorical Algebra and Calculus

Multi-model databases are designed to store, manage, and query data in various models, such as relational, hierarchical, and graph data, simultaneously. In this paper, we provide a theoretical basis for querying categorical databases. We propose two formal query languages: categorical calculus and categorical algebra, by extending relational calculus and relational algebra respectively. We demonstrate the equivalence between these two languages of queries. We propose a series of transformation rules of categorical algebra to facilitate query optimization. Finally, we analyze the expressive power and computation complexity for the proposed query languages.

==> algorithms/closureFD.tex <==
\KwIn{A graph representation $G$ and  a set of functional dependencies $F$ } 
\KwOut{The relevant closure representation  $(G,F)^+$} 
\DontPrintSemicolon

 Convert $G$ to a set of functional dependencies denoted by $FD(G)$;
 
 $D = FD(G) \cup F$;
 
\ForEach{  $X \in LHS(D)$} 
{
    \If{$X \notin G$}
        {
        add $X$ in G; 
        }
    
    Compute the closure attributes of $X$: giving $X^+$;

   \ForEach{  $Y \in X^+$ and $Y \in G$} 
    {
     \If{ there is no arrow from $X$ to $Y$ in $G$}
        {
        add an arrow from $X$ to $Y$ in $G$;
        }
    }
    
        
}


==> algorithms/closureMVD.tex <==
\KwIn{A graph representation $G$, a set of functional dependencies $F$ and a set of multivalued dependencies $M$} 
\KwOut{The relevant closure representation of $(G,F,M)^+$} 
\DontPrintSemicolon

 Convert $G$ to a set of functional dependencies denoted by $FD(G)$;
 
$D$ = $FD(G) \cup F \cup M$;
 
\ForEach{  $X \in LHS(D)$} 
{
        \If{$X \notin G$}
        {
        add $X$ in $G$;
        }
        

        Compute the FD closure attributes of $X$ based on $D$: giving $X^+$;

        \ForEach{  $Y \in X^+$ and $Y \in G$} 
        {
            \If{$X \to Y $ is not an arrow in $G$}
            {
            add an arrow from $X$ to $Y$ in $G$;
            }
        }

       Identify all MVD objects in $G$ based on the inferred MVDs from $D$;
}


==> algorithms/compute1RR2.tex <==
\KwIn{A graph representation $G$ and  a set of functional dependencies $F$} 
\KwOut{The first reduced representation of $G$} 
\DontPrintSemicolon

 Use Algorithm \ref{alg:closureFD} to compute a closure graph $(G,F)^+$;

\ForEach {arrow  $f: X \to Y$ in $(G,F)^+$} 
{
    \If{($(G,F)^+ - f)$ is equivalent to $(G,F)^+$}
    {
    Remove $f$ in $(G,F)^+$;
    }
}

Return the updated graph $(G,F)^+$;







==> algorithms/compute2RR.tex <==
\KwIn{A graph representation $G$, a set of multivalued dependencies $M$ and  a set of functional dependencies $F$} 
\KwOut{The second reduced representation (2RR) of $G$} 
\DontPrintSemicolon


 Use Algorithm \ref{alg:closureMVD} to compute a closure graph $(G,F,M)^+$;

% $D = FD(G') \cup M$ \tcp*{FD(G') is a set of FDs in G' }

$G'=$\texttt{Remove\_Objects}($(G,F,M)^+$);




\ForEach {arrow  $f: X \to Y$ in $G'$} 
{
    \If{($G' - f$) is equivalent to $G'$}
    {
    Remove $f$ in $G'$;
    }
}

Return the updated $G'$;

%Step 4: Compute a minimal cover V of FDs for $G_3$

%FOREACH object X remove all associated and composed FDs in ClosureFD(X)+ ENDFOR

%Step 5: Generate a graph representation $G_4$ based on  $V$ 



\SetKwFunction{func}{ $\mbox{Remove\_Objects}$}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\func{$G$}}
{
%Convert $G$ to a set of FDs, denoted by $FD(G)$

%Compute the dependent basis of MVD in $FD(G) \cup M$ \tcp*{Appendix for details}

\While{$\exists$ any derivable MVD object $O \in G$ w.r.t $X \to\to_O Y$ }
 {
    decompose $O$ into two objects $O_1= X \cup Y$ and $O_2=O-Y$ and assign the corresponding projection arrows for $O_1$ and $O_2$;

    %\ForEach{projection arrow $f:O \to N$ }
    %    {
    %        \If{$\pi(N) \subseteq \pi(O_i)$ (i=1 or 2)}
     %        {
     %           add the projection arrow $f':O_i \to N$
     %       }
     %   }
    
  }

  Remove all derivable limit  objects in $G$; 

  
  Return the updated $G$;
}





%Compute the minimal cover C of $FD(G) \cup M \cup F$

%while there is a MVD in C but not in an object in G

%add one new object for this MVD, ENDHILE

%Continue to use the 1RR computation algorithm for G with functional dependencies and multivalued dependencies. 






==> algorithms/map2DTD2.tex <==
\KwIn{A graph representation $\mathcal{G(C)}$ of a schema of a category $\mathcal{C}$ }
    \KwOut{XML DTD $\mathcal{D}$=($L$, T, P, R, r)}
    \DontPrintSemicolon

Let $\epsilon$ be the root $r$ of $D$;

 $T= \{@ID\}$;

 Initialize $L$, $P$, and $R$ to be empty sets;

\ForEach{ unprocessed object $O$ in $V(\mathcal{G(C)})$ with outgoing edges}
{ 
     $L \leftarrow L \cup \{\lambda(O)\}$; \tcp*{$\lambda(O)$ is the label of $O$}

     $P_\epsilon \leftarrow P_\epsilon \cdot (\lambda(O))^+$;
    
     $R(\lambda(O))=\{@ID\}$;
    
    Add\_neighbours($O$);
      
    %Process\_entities\_relationships($O$)

     Mark $O$ as a processed node;
    
}


\SetKwFunction{func}{ $\mbox{Add\_neighbours}$}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\func{$O$}}
{
    \ForEach{unprocessed object $N$ in $outNbr(O)$ }
    {    
     \If{$N$ has any outgoing edge}
     { 
        $T= T \cup \{@\lambda(N)$\_ID\};
        
        $R(O)=R(O) \cup \{@\lambda(N)$\_ID\};
     }
    \Else 
     {  
       $P_O \leftarrow P_O \cdot \lambda(N)$;

        $L \leftarrow L \cup \{\lambda(N)\}$;
      }   
    }
}   




==> algorithms/map2propertygraph2.tex <==
\KwIn{A graph representation $\mathcal{G(C)}$ of schema of a category $\mathcal{C}$ }
    \KwOut{A property graph  schema $\mathcal{PG}$= ($V, E, T, P$)}
    \DontPrintSemicolon

Initialize $V, E, T$, and $P$ to be empty sets;

\ForEach{ object $O$ in $V(\mathcal{G(C)})$ with outgoing edges}
{
     $V \leftarrow V \cup \{\lambda(O)\}$;

     \If{$O$ is an entity or attribute object  }
     {
        $P(O) \leftarrow P(O) \cup \{SK\}$;
     }
    
     Add\_neighbours($O$);
     
    %Process\_attributes($O$) 

    %Process\_entities\_relationships($O$)

    %Process\_relationships($O$)

    Mark $O$ as a processed object; 

}



\SetKwFunction{func}{ $\mbox{Add\_neighbours}$}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\func{$O$}}
{
    \ForEach{ object $N$ in $outNbr(O)$ }
    {
        \If{$N$ is an attribute object and $N$ has no outgoing edges} 
        { 
            $P(O) \leftarrow P(O) \cup \{\lambda(N)\}$; 

            $T \leftarrow T \cup \{\lambda(N)\}$; 
        }
        \Else
        { 
            $E \leftarrow E \cup \{(O,N)\}$;

          %  $V \leftarrow V \cup \{N\}$
            
           % $P((O)) \leftarrow P((O)) \cup \{IDREF\}$
      
        }
         
        
        %\If{$N \in bin(O)$} 
        %{ 
        
        %    Add\_neighbours($N,S$)

        %    Mark $N$ as a processed object

        %}

        
        
    }
    
}   

%\SetKwFunction{func}{ %$\mbox{Process\_entities\_relationship}$}
%\SetKwProg{Fn}{Function}{:}{}
%\Fn{\func{$O$}}
%{
%    \ForEach{entity or relationship object $N$ in $outNbr(O)$ }
%    {
        
        %Create an edge $e$ between $N$ and $O$ and add $e$ into $E$ in schema

        %$E \leftarrow E \cup \{(N,O)\}$

        %$P((N)) \leftarrow P((N)) \cup \{ID\}$

        %$P((O)) \leftarrow P((O)) \cup \{IDREF\}$
     
        
    %}
%}

%\SetKwFunction{func}{ $\mbox{Process\_relationships}$}
%\SetKwProg{Fn}{Function}{:}{}
%\Fn{\func{$O$}}
%{
%    \ForEach{relationship object $R$ in $outNbr(O)$ }
%    {
            
%        \If{R is a binary relationship object} 
%        {
%            $P(R) \leftarrow P(R) \cup \{N \}$   
%        }
%        \Else 
%        {
            %create an edge $e$ between $R$ and $O$ into $E$ in the schema

%            $E \leftarrow E \cup \{(R,O)\}$
                
%        }
            
        
%    }
%}

==> algorithms/map2relationschema3.tex <==
\KwIn{A reduced graph representation $G(C)$ of  a schema category $\mathcal{C}$ }
\KwOut{Relation schema   $\mathcal{R}$=\{$R_1,R_2,...,R_p$\}}
\DontPrintSemicolon

\ForEach{ unprocessed object $O_i$ in $V(G\mathcal{(C)})$ with outgoing edges } 
{
    Create a table $R_i$ for $O_i$; \tcp*{$i$=1,...,$p$}

    \If{ $O_i$ is a relational or entity object} 
    { 
        $sort(R_i) = \{SK\}$; \tcp*{Surrogate Key}
    }
    \Else{
        $sort(R_i) = \{\lambda(O_i)\}$; \tcp*{$\lambda(O_i)$ is the name of the object $O_i$}
    }

    Add\_neighbours($R_i,O_i$);

    Mark $O_i$ as a processed object;

}

 Clean($\mathcal{R}$);


\SetKwFunction{func}{ $\mbox{Add\_neighbours}$}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\func{$R,O$}}
{
    \ForEach{object $N$ in $outNbr(O)$ }
    {
         
        %Add an attribute $\lambda(f)$ in relation $R_i$ 

        $sort(R) \leftarrow sort(R) \cup \{\lambda(N)\}$;

        \If{$N$ is a relational or entity object} 
        { 
        Let $\lambda(N)$ be a foreign key in $R$ to reference to $SK$ in $N$; 
        }
        
        \If{ $N \in bin(O)$} 
        { 
            Add\_neighbours($R,N$);   \tcp*{Add the outgoing neighbours of $N$ into $R$}

            Mark $N$ as a processed object;
        }
    }
}   


\SetKwFunction{func}{ $\mbox{Clean}$}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\func{$\mathcal{R}$}}
{
    \ForEach{relation $R_i$ in $\mathcal{R}$ }
        {\If{$K$ is the surrogate key without any referential from other relations} 
            { 
              Remove $K$ in $R_i$; 
         } 
    }

    \If{$sort(R_i) \subseteq sort(R_j)$ in $\mathcal{R}$} 
            { 
                Remove $R_i$ in $\mathcal{R}$; 
            } 
        
}

==> equivalence.tex <==
\section{Proof of equivalence theorem between categorical calculus and algebra}

The objective of this section is to show the equivalence between categorical algebra and categorical calculus. 

 \smallskip


\noindent \textbf{Theorem}
\ref{the:equivalent}.  \textit{The categorical calculus  and categorical algebra are equivalent.}   

\smallskip

Proof: The proof can be accomplished using the following two steps:


(i) Algebra queries $\sqsubseteq$ calculus queries; and

(ii) Calculus queries $\sqsubseteq$ algebra queries.

For (i) it is sufficient to show that each of the algebraic operations can be simulated by a calculus expression. The simulation of algebra operations by calculus expression is as follows:

1. Map $f(S_1)$, $f: S_1 \to S_2$ : \[ \{y | y \in S_2 \wedge \exists x \in S_1, y = f(x) \}; \]

2.  Select  $\sigma_{A \theta_M B}(S)$: \[ \{x |x \in S \wedge A(x) \theta_M B(x) \} \]


3. Project $\pi_A R$, where $A= A_1,...,A_k$ is a sublist of components of a relationship object $R$.  \[ \pi_A R = \{ (x_1,...,x_k) |  x_i \in A_i (1 \leq i \leq k) \wedge \exists (x_1,...,x_k,x_{k+1},..., x_n) \in  R \}\]



4. $S_1[A] \div S_2[B]$: \[ \{ (x_1,\ldots,x_n) |  (x_1, \ldots, x_n) \in \pi_{\overline{A}} S_1  \wedge (\forall (y_1, \ldots, y_m) \in  \pi_{B} S_2´,  (x_1, \ldots, x_n, y_1, \ldots, y_m) \in S_1)  \}\]

5. $getParent$($D_1$, $D_2$), where  $D_1$ and $D_2$ are two Dewey code sets.  \[ \{(x_1,x_2) | x_1 \in D_1 \wedge x_2 \in D_2 \wedge x_1 ~ isParent ~ x_2\} \]

%The simulation of other tree operators can be found in Appendix \ref{sec:otheralgebra}.

6. $getReach(S,T,E)$, where $S$ and $T$ denote the source and target node set, and $E$ the edge set. \[ \{(x_1,x_2) | x_1 \in ~ S \wedge x_2 \in ~ T \wedge x_1  \rightsquigarrow^E x_2  \}; \]


7. $getnHop$($S,T,E$):  \[ \{(x_1,x_2) | x_1 \in ~ S \wedge x_2 \in ~ T \wedge x_1 \rightsquigarrow_n^E x_2  \};
\]


%6. $S_1 \cup S_2$ corresponds to $\{x | x \in S_1 \vee  x \in S_2  \}$

%7. $S_1 \cup S_2$ corresponds to $\{x | x \in S_1 \wedge  x \in S_2  \}$

%8. $S_1 - S_2$ corresponds to $\{x | x \in S_1 \wedge  x \notin S_2  \}$

%9. $S_1 \times S_2$ corresponds to $\{r | \exists x_1, x_2, \pi_1(r)=x_1 \wedge \pi_2(r)=x_2  \}$



8. $Cat(S_1,\cdots,S_n, f_1: S_{i_1} \to S_{j_1},\cdots,f_m: S_{i_m} \to S_{j_m})$: \[ \{x_1,\ldots,x_n | x_i \in S_i (1 \leq i \leq n) \wedge f_k:S_{i_k} \to S_{j_k}(1 \leq k \leq m) \} \]

9. $Lim(Cat(S_1,\cdots,S_n, f_1:S_{i_1} \to S_{j_1},\cdots, f_m: S_{i_m} \to S_{j_m}))$: \[ \{(x_1, \cdots , x_n) |  x_i \in S_i (1 \leq i \leq n) \wedge f_{k}(x_{i_k}) = x_{j_k} (1 \leq k \leq m)  \} \]


%\[  \{(x_1, \cdots , x_n)| \forall x_i \in S_i (1 \leq i \leq n), \forall f_k: x_{i_k} \to x_{j_k}, f(x_{i_k})=x_{j_k} (1 \leq k \leq m) \}  \]

\smallskip

Then we proceed to prove that (ii) calculus queries $\sqsubseteq$ algebra queries.

%The reduction algorithm would be roughly as follows: First, the categorical calculus expression is converted into prenex normal form and disjunctive normal form. Second, for each conjunctive conjunction, a category is constructed to include all variables and their associated morphisms.   Third, a limit of ´each category is computed and elements that do not satisfy the communicative diagram of the limit are naturally removed. Fourth, the remaining elements in the limit are whittled down by further selection and division. Finally, the target objects and morphisms are categorized to generate the desired result. A more formal and detailed account follows.


We will exhibit an algorithm for translating a calculus expression into a semantically equivalent algebraic expression. The reduction algorithm can be outlined as follows: First, the categorical calculus expression is converted into prenex normal form where the quantifier-free part (matrix) is disjunctive normal form. Second, for each conjunctive clause, a category is constructed to include all variables and their associated morphisms. Third, the limit of each category is computed, and elements that do not satisfy the commutative diagram of the limit are naturally removed. Fourth, the remaining elements in the limit are further refined through selection and division. Finally, the target objects and morphisms are projected to construct the desired result. A  detailed account follows.


Step 1: 

(1.1) Convert $V$ to the prenex normal form without expanding the range-coupled qualifiers;

(1.2) Convert the matrix (the part of the formula that remains after all quantifiers) in $V$ into disjunctive normal form;

(1.3)  Apply a change to variables resulting from (1.2) so that variables become $x_1$,...,$x_{n}$ in the order of their first occurrence in the qualification. 

%Note that the first occurrence of a bounded variable is with its quantifier.



Let a calculus expression resulting from the above transformations be 

\vspace{-4mm}
\[ Z' = \{  X', \mathcal{R'} | U' \wedge F'  \wedge V' \} \]

%Assume taht There are $m+q$ element variables in $X$ and $R$. Let the quantifier ($\exists$ or $\forall$ ) associated with $r_j$ in V' be $Q_j$, and let the proper range term over $r_j$ in V' be $U'_j$. 



Step 2: Generate the following three types of objects and morphisms;

(2.1) Generate entity or attribute objects for each variable in $X'$ and $\mathcal{R'}$, For each variable $x_i$, form a defining equation of the range term of  $x_i$. The algebraic expression on the right-hand side of this equation is obtained by applying the following rewriting rules to $x_i$:

(i) $ x_i \in O \Rightarrow S_i = O$
(ii) $\vee \Rightarrow \cup$ (set union)
(iii) $\wedge \Rightarrow \cap$ (set intersection)
(iv) $\wedge \neg \Rightarrow -$

For example, if $x_i \in O_1 \wedge  \neg x_i \in O_2$, then the defining equation for $S_i$, 
\vspace{-1mm}
\[ S_i = O_1-O_2\]

In this case, $O_1$ and $O_2$ must be union-compatible. 

%(2.2) Generate the new relationship objects $R_1,...,R_n$ with the associated object components and the morphisms. Assume $R_i=(x_{i_1},\cdots,x_{i_m})$, then create an objects $R_i$ and the associated projected morphisms $\pi_j: R_i \to X_{i_j}$ $( 1 \leq j \leq m)$.     


(2.2) Generate relationship objects for each set $R_i$ of variables in $\mathcal{R'}$. Specifically, for each \( R_i = (x_{i_1}, \ldots, x_{i_m}) \), create objects \( R_i \) and define the associated projected morphisms \( \pi_j: R_i \to S_{i_j} \) for each \( j \) (\( 1 \leq j \leq m \)) where $x_{i_j} \in S_{i_j}$.  

(2.3) Generate relationship objects for all tree and graph predicates in $V'$, including reachable ($\rightsquigarrow^E$), nHop ($\rightsquigarrow_n^E$), $isParent$, and other tree operators.

(i)  $x_1 \in S, x_2 \in T, x_1 \rightsquigarrow^E x_2$ $\Rightarrow$  Create $R_i = getReach(S,T,E)$, $\pi_1: R_i \to S$ and $\pi_2: R_i \to T$;

(ii) $x_1 \in S, x_2 \in T, x_1 \rightsquigarrow^E_n x_2$ $\Rightarrow$  Create $R_i = getnHop(S,T,E)$, $\pi_1: R_i \to S$ and $\pi_2: R_i \to T$;

(iii) $x_1 \in D_1, x_2 \in D_2, isParent(D_1,D_2)$ $\Rightarrow$ Create $R_i = getParent(D_1,D_2)$, $\pi_1: R_i \to D_1$, $\pi_2: R_i \to D_2$.



Step 3: 

(3.1) For each clause $C_k$ in the disjunctive normal form of $V'$, generate morphisms such that ($f(x_i)=x_j$ or $x_i \cdot S_j = x_j$) $\Rightarrow f: S_i \to S_j$, where $x_i$ and $x_j$ appear in the clause $C_k$.

(3.2) Construct one category $ \mathcal{C}_k$ for each clause, involving the associated objects and morphisms from Steps (2) and (3.1), $ \mathcal{C}_k= Cat(S_1,\cdots,S_n, f_1:S_{i_1} \to S_{j_1},\cdots, f_m: S_{i_m} \to S_{j_m})$;

(3.3) Compute a universal limit object $L_k = Lim(Cat(\mathcal{C}_k)$, where   $\mathcal{C}_k$ is the category in Step (3.2).

Step 4: For each clause $C_k$ in the disjunctive normal form of $V'$, continue to apply the select operations for each limit object $L_k$ generated from step (3).


(i) $A(x_i) \theta_M  B(x_j) \Rightarrow \sigma_{A(x_i) \theta_M  B(x_j) }(L_k)$
(ii) $A(x_i) \theta_M  \alpha \Rightarrow \sigma_{A(x_i) \theta_M  \alpha }(L_k)$

where $a$ is an individual constant, $\theta_M$ is one of $=,\neq,>,<,\leq,\geq$. 

%Note that the symbol $\neg$ does not occur at all here due to the transformation in step 1.

%Step 5: Compute the division on the limit object from the above step to reflect $S_j$'s ($1 \leq j \leq n$) which have the effect of the universal quantifier $\forall$ of $V'$. The division is  $L[S_1,\cdots,S_n] \div (S_1 \times \cdots \times S_n)[S_1,\cdots,S_n] $, where $L$ is the limit object from Step 4, $S_1 \times \cdots \times S_n$ denotes the Cartesian product  of sets. After the division for each clause,  union the results from individual clause.

Step 5: Compute the division on the limit object obtained in the previous step to incorporate \( S_j \) ($ 1 \leq j \leq n $) corresponding to the universal quantifier \( \forall \) of \( V' \). The division operation is defined as \( L[S_1,\cdots,S_n] \div (S_1 \times \cdots \times S_n)[S_1,\cdots,S_n] \), where \( L \) represents the limit object from Step (4), and \( S_1 \times \cdots \times S_n \) denotes the Cartesian product of sets. After performing division for each clause, combine the results from individual clauses using a union operation.



Step 6:  Form projected objects that take into account the target objects in $X'$ and $\mathcal{R'}$. Finally, construct the desired target category.

%with those projected objects (including entity, attribute and relationship objects from $X$ and $R$) and the associated morphisms in $F'$.

%Refer to the category schema in Figure \ref{fig:SC2}(a). Consider the following query: find the addresses of all male students who attend every course attended by at least one female student. . The categorical calculus expression for this query is:


The validity of the reduction algorithms relies on the following lemmas. 

%\begin{lemma} This lemma proves the validity of step 4 about the construction of a category and the computation of the limit. Let $x$ be a returned variable, assume that $x \in S_x$ and $y \in S_y$, and $f: S_x \to S_y$. Then\[\{ x: f(x) = y \} = \pi_x (Lim(S_x,S_y,f: S_x \to S_y))\]\end{lemma}

\begin{lemma}\label{lem:R} Consider a category $\mathcal{C}$ with a set of objects $S_1, S_2, \cdots, S_n$ and  functions $f_1:S_1 \to S_2, \cdots, f_n:S_n \to S_{n+1}$. Let a relational object $R=Lim(\mathcal{C})$. We have $\forall x_i \in \pi_{S_i} (R)$, $f(x_i) \in S_{i+1}$, where $1 \leq i \leq n$.
\end{lemma}

\begin{proof}
Based on the definition of limit operator in Section \ref{sec:sublimit}: 
\[R =  \{(x_1, x_2, \cdots, x_{n+1} )|  x_1 \in S_1, \cdots, x_{n+1} \in S_{n+1}   \wedge   f(x_{1})=x_{2}, \cdots, f(x_{n})=x_{n+1} \}\]

Therefore,  $\pi_{S_i} (R) = S_i$ and $\forall x_i \in S_i $, $f(x_i) =x_{n+1} \in S_{n+1}$, where $1 \leq i \leq n$.

\end{proof}


%\begin{proof}Based on the definition of limit operator in Section \ref{sec:sublimit}: \[R =  \{(x_1, x_2, \cdots, x_{n+1} )|  x_1 \in S_1, \cdots, x_{n+1} \in S_{n+1}   \wedge   f(x_{1})=x_{2}, \cdots, f(x_{n})=x_{n+1} \}\]Therefore,  $\pi_{S_i} (R) = S_i$ and $\forall x_i \in S_i $, $f(x_i) =x_{n+1} \in S_{n+1}$, where $1 \leq i \leq n$.\end{proof}

\begin{lemma}\label{lem:division} This lemma addresses the validity of the computation of division for multiple  $\forall$ quantifiers. Consider the following calculus expression: \begin{equation}
\begin{split}
\{ x_1 | x_1 \in S_1  \wedge \forall y_1 \in S_2,  \cdots, \forall y_n \in S_{n+1}, \exists z_1 \in R_1, \cdots, \exists z_n \in R_n, f_1(z_1)=x_1 \wedge  g_1(z_1)=y_1,  \\
              \cdots \wedge f_n(z_n)=x_n \wedge g_n(z_n)=y_n \}
\end{split}
\end{equation}

This expression is equivalent to the following algebraic operators: \[\pi_{S_1}(L[S_2,S_3, \cdots, S_{n+1}] \div (S_2 \times S_3 \times \cdots S_{n+1} )[S_2,S_3 \cdots, S_{n+1}])\]  where $L=Lim(Cat(S_1,\cdots,S_{n+1},R_1, \cdots, R_n,f_1:S_1 \to S_2, \cdots, f_n:S_1 \to S_{n+1}))$.

\end{lemma}



\begin{proof}
Based on the definition of division operator in Section \ref{sec:divisiontree},

$\pi_{S_1}(L[S_2,S_3, \cdots, S_{n+1} ] \div (S_2 \times S_3 \times \cdots S_{n+1} )[S_2,S_3, \cdots, S_{n+1}])$ returns \[ \{ x_1 | x_1 \in S_1 \wedge  \exists z_1 \in R_1, \cdots, \exists z_n \in R_n, \forall (y_1, y_2, \cdots, y_{n}) \in  \pi_{S_2,S_3, \cdots, S_{n+1}}(R),  (x_1, y_1, \cdots, y_{n}, z_1, \cdots, z_n ) \in R  \}\]

Note that $L$ is a limit object computed through the category $\mathcal{C}$=$Cat$($S_1,\cdots,S_{n+1},R_1, \cdots, R_n,f_1:S_1 \to S_2, \cdots, f_n:S_1 \to S_{n+1}$). Thus, based on Lemma \ref{lem:R},  the above expression can be rewritten as 
$\{ x_1 | x_1 \in S_1  \wedge \forall y_1 \in S_2, \cdots, \forall y_n \in S_{n+1}, \exists z_1 \in R_1, \cdots, \exists z_n \in R_n,  f_1(z_1)=x_1 \wedge  g_1(z_1)=y_1,$ $\cdots \wedge f_n(z_n)=x_n \wedge g_n(z_n)=y_n \}$, as desired. 


\end{proof}


\begin{lemma}\label{lem:graphoperator} This lemma addresses the validity of the reachability operator for graph data. Consider the following calculus expression: $\{ x_1, x_2 | x_1 \in S_1  \wedge x_2 \in S_2  \wedge x_1 \rightsquigarrow^E x_2 \wedge \exists x_3 \in S_3, f_1(x_3)=x_1 \wedge f_2(x_3)=x_2\}$. This calculus can be implemented with the following three algebraic operators: $S_4$= $getReach(S_1,S_2,E)$; $S_5$ =  $Lim(Cat(S_1,S_2,S_3,S_4,f_1: S_3 \to S_1,f_2: S_3 \to S_2,\pi_1: S_4 \to S_1,\pi_2: S_4 \to S_2))$ and $S_6$ = $\pi_{S_1,S_2}S_5$. 
\end{lemma}


\begin{proof}
The $getReach$ operator returns the pairs of elements from $S$ and $T$ which are reachable via the edges in $E$. 

$S_4$= $\{ x_1, x_2 | x_1 \in S  \wedge x_2 \in T  \wedge x_1 \rightsquigarrow^E x_2 \}$,

Based on the definition of limit operator in Section \ref{sec:sublimit}: 
\[S_5 =  \{(x_1, x_2,x_3, x_4 )|  x_1 \in S_1, x_2 \in S_2, x_3 \in S_3, x_4 \in S_4,   f_1(x_{3})=x_{1} \wedge f_2(x_{3})=x_{2} \wedge \pi_{S_1}(x_{4})=x_{1} \wedge \pi_{S_2}(x_{4})=x_{2} \}\]

Apply the definition of the reachability predicate: \[S_5 =  \{(x_1, x_2,x_3, x_4 )|  x_1 \in S_1, x_2 \in S_2, x_3 \in S_3, x_4 \in S_4,   f_1(x_{3})=x_{1} \wedge f_2(x_{3})=x_{2} \wedge (x_1 \rightsquigarrow^E x_2) \}\]

Finally, perform the projection operator on $x_1$ and $x_2$: \[S_6 =  \{(x_1, x_2 )|  x_1 \in S_1, x_2 \in S_2,  \exists x_3 \in S_3, f_1(x_{3})=x_{1} \wedge f_2(x_{3})=x_{2} \wedge (x_1 \rightsquigarrow^E x_2) \}\]

as desired.

\end{proof}

Theorem \ref{the:express}: \textit{ Categorical  calculus and categorical algebra can express all of the following:
    \begin{itemize}
        \item Relational calculus and algebra queries;
        \item Graph pattern matching and graph reachability queries;
        \item XML twig pattern queries. 
    \end{itemize}}
    


\noindent \textbf{Proof}: (Sketch) Categorical algebra contains the main operations found in relational algebra, making it capable of expressing any relational query. The fundamental operations in relational algebra—\textit{Select}, \textit{Project}, \textit{Cartesian Product}, \textit{Union}, and \textit{Set Difference}—each have corresponding counterparts in categorical algebra. Note that Cartesian product is a specific instance of the \textit{limit} operator, in the case of the absence of morphisms between objects. Further, graph reachability can be addressed using reachable ($\rightsquigarrow^E$ and $\rightsquigarrow_n^E$) predicates, while graph pattern matching can be translated into \textit{Map}, \textit{Select}, and \textit{Limit} operators to find all matching nodes. Moreover, parent-child, ancestor-descendant, sibling and other tree relationships can also be implemented using the corresponding categorical predicates with the assistance of Dewey codes of XML elements.


\smallskip

Theorem \ref{the:complexity}: \textit{
Consider a category $\mathcal{C}$ with $p$ objects and $q$ morphisms. Let the maximum number of elements in any object of $\mathcal{C}$ be $n$.
}
\begin{enumerate}
    \item The data time complexity of computations for categorical calculus and categorical algebra in $\mathcal{C}$ is bounded by $O(q \cdot n^p)$.
    \item The space complexity of these computations is bounded by $\text{NSPACE}[\log n]$.
\end{enumerate}


\noindent \textbf{Proof}: Due to the equivalence between categorical calculus and categorical algebra, we analyze the time complexity of categorical algebra. The main operators are analyzed as follows:

(1) Map $f(S)$: the time complexity is $O(n)$, where $n$ denotes the number of elements in  $S$; 

(2) Project $\pi(R)$: the time complexity is $O(n log(n))$, where $n$ denotes the number of elements in $R$, as this operator requires the removal of the duplicate elements; 

(3) Select $\sigma_C(S)$:  the time complexity is $O(n)$, where $n$ denotes the number of elements in  $S$; 

(4) $getParent(D_1,D_2)$:  the time complexity is $O(|D_1| \cdot |D_2|)$;

(5) $getReach(S,T,E)$:  the time complexity is O($n^2$+$min(|S|, |T|) \cdot |E|$) time, where $n$ is the total number of nodes in the graph, as shown in Algorithm \ref{alg:OTC}.

(6) $Lim(\mathcal{C})$: assuming that the category $\mathcal{C}$ contains $p$ objects, $q$ morphisms and the maximum number of elements in one object is $n$. The total cost is $O(q \cdot n^p)$ in the worst case.




The most computationally expensive operator in the list above is \( Lim(\mathcal{C}) \). If an algebraic query involves \( k \) operators, the total computational cost is \( O(k \cdot q \cdot n^p) \). Given that \( k \) is typically small relative to other parameters in the dataset, the data complexity simplifies to \( O(q \cdot n^p) \).


Regarding space complexity, most operators, except for the $getReach$ operator, operate within LOGSPACE, similar to relational calculus. However, the $getReach$ query has a space complexity of \( O(\log^2 n) \), comparable to transitive closure \cite{10.1145/800141.804682}. Consequently, the overall space complexity of the operators falls under NSPACE[\(\log n\)].





==> relatedwork.tex <==
\section{Related work}



This work is related to two categories of previous research: (1) applied category theory for query languages in databases, and (2) query calculus and algebra for various types of data.

\smallskip

\noindent \textbf{Applied category theory for query languages}. Although category theory was initially developed as an abstract mathematical language to unify algebra and topology, researchers have explored its applications in various fields, including database query languages. Tannen (1994) \cite{conf/pods/Tannen94} highlights that concepts from category theory can lead to a series of useful languages for collection types such as sets, bags, lists, complex objects, nested relations, arrays, and certain kinds of trees.  Libkin (1995) \cite{DBLP:conf/icdt/Libkin95} uses universality properties to study the syntax of query languages with approximations. Libkin and Wong (1997) \cite{journals/jcss/LibkinW97} showcase the connection between database operations on collections and the categorical notion of a monad. More recently, Schultz and Spivak (2016) \cite{schultz2016algebraic} introduce a categorical query language that serves as a data integration scripting language. Gibbons et al. (2018) \cite{journals/pacmpl/GibbonsHHW18} present an elegant mathematical foundation for database query language design using category theory concepts such as monads and adjunctions. These works demonstrate the intriguing connections between category theory and query languages and query processing, revealing how category theory can inform and enhance database query language design.




%Although category theory was developed as an abstract mathematical language to unify algebra and topology, researchers tried to apply it in different fields. To apply category theory on database query languages, Tannen (1994) \cite{conf/pods/Tannen94} highlights that category theory concepts lead to a succession of useful languages that includes equivalents of familiar languages for relational databases, such as relational algebra, nested relational algebra and datalog.   Libkin (1995) \cite{DBLP:conf/icdt/Libkin95} uses universality properties to study syntax for query languages with approximations.  Libkin and Wong (1997) \cite{journals/jcss/LibkinW97} showcasing the connection between database operations on collections with the categorical notion of a monad. Recently, Schultz and Spivak \cite{schultz2016algebraic}(2016) show a categorical query language. which is a data integration scripting language.   Gibbons et al. (2018) \cite{journals/pacmpl/GibbonsHHW18} shows an elegant mathematical foundation for database query language design with the concepts of category theory  such as monad and adjunctions.  These previous papers demonstrate the interesting connection between some concepts of category theory with query languages and query processing. 

%They show that some open problems in the field of data sharing in computational science are addressable by working within this paradigm of functorial data migration.

\smallskip

\noindent \textbf{Query calculus and algebra.}  Since Codd (1972)  \cite{DBLP:persons/Codd72} demonstrated that the same class of database queries can be expressed by relational algebra and the safe formulas of relational calculus, query algebra and calculus have become central topics in database research. A plethora of related works exist on query algebra and calculus across various types of data, including 
relational data \cite{DBLP:persons/Codd72,10.1145/114325.103712,10.1145/99935.99943,10.1145/32204.32219}, nested relational data \cite{DBLP:conf/pods/ParedaensG88,DBLP:conf/pods/Gucht87}, graph data \cite{DBLP:conf/pods/FrancisGGLMMMPR23,10.1093/comjnl/bxaa031}, object-oriented data \cite{10.1145/588011.588026}, incomplete and probabilistic data \cite{suciu:OASIcs.Tannen.10,10.1145/1265530.1265535}, etc. These previous papers lay the foundation for database systems to process various types of data. Our paper makes contributions by proposing query calculus and algebra for categorical data with the application on multi-model databases.

%\begin{itemize}\item Relation data: Codd  \cite{DBLP:persons/Codd72} proposed relational calculus and algebra and show their equivalence. \item Graph data:  Francis et al. \cite{DBLP:conf/pods/FrancisGGLMMMPR23} proposes a simple Graph Pattern Calculus (GPC) that reflects all the key pattern matching features of GQL and SQL/PGQ. We describe the syntax and semantics of GPC, along with the typing rules that ensure its expression  Paper \cite{10.1093/comjnl/bxaa031} proposes a semi-join algebra for graph query optimization.\item  Object-oriented data: Related work \cite{10.1145/588011.588026}  on OODB calculus and algebra: Some papers propose object-oriented calculus, which incorporates object-oriented components such as QID, different notions of equality, and method calls. \item Incomplete and probabilistic data: Related work on algebra calculations for incomplete databases and probabilistic databases \cite{suciu:OASIcs.Tannen.10}. Paper  \cite{10.1145/1265530.1265535} introduces K-relations in which tuples are annotated with elements from K. They define a generalized positive algebra on K-relations and argue that K must be a commutative semiring.\end{itemize}





